ATLASv2: LLM-Guided Adaptive Landmark Acquisition and Navigation on the Edge

Autonomous systems deployed on edge devices face significant challenges, including resource constraints, real-time processing demands, and adapting to dynamic environments. This work introduces ATLASv2, a novel system that integrates a fine-tuned TinyLLM, real-time object detection, and efficient path planning to enable hierarchical, multi-task navigation and manipulation all on the edge device, Jetson Nano. ATLASv2 dynamically expands its navigable landmarks by detecting and localizing objects in the environment which are saved to its internal knowledge base to be used for future task execution. We evaluate ATLASv2 in real-world environments, including a handcrafted home and office setting constructed with diverse objects and landmarks. Results show that ATLASv2 effectively interprets natural language instructions, decomposes them into low-level actions, and executes tasks with high success rates. By leveraging generative AI in a fully on-board framework, ATLASv2 achieves optimized resource utilization with minimal prompting latency and power consumption, bridging the gap between simulated environments and real-world applications.

==> sections/tables_and_figures/LLM_evaluation.tex <==
% \begin{table*}[t]
% \centering
% \caption{Comparison of correct task responses for a Cloud Chat GPT 4 LLM, Pre-trained TinyLLama LLM post Q5\_K medium quantization, and Fine-tuned TinyLLama post Q5\_K medium quantization and fine tuning across two simulated environments. The table highlights the performance of each model in interpreting and executing natural language prompts for navigation and object interaction tasks. Scores are shown as successful number of subtasks out of the expected number of subtasks for each prompt, with the overall performance summarized at the bottom. Results are shown for objects and locations present in the knowledge base and prompt header.}
% \begin{tabular}{|cccc|}
% \hline
% \multicolumn{4}{|c|}{\textbf{ENVIRONMENT 1}}                                                                                                                                                                                                                              \\ \hline
% \multicolumn{1}{|c|}{\textbf{Prompt}}                                                                                                                & \multicolumn{1}{c|}{\textbf{Cloud LLM}} & \multicolumn{1}{c|}{\textbf{Pre-trained  LLM}} & \textbf{Fine-Tuned LLM} \\ \hline
% \multicolumn{1}{|c|}{\textit{Navigate to Room 1}}                                                                                                    & \multicolumn{1}{c|}{1/1}                & \multicolumn{1}{c|}{0/1}                       & 1/1                     \\ \hline
% \multicolumn{1}{|c|}{\textit{Navigate to Room 2}}                                                                                                    & \multicolumn{1}{c|}{1/1}                & \multicolumn{1}{c|}{0/1}                       & 1/1                     \\ \hline
% \multicolumn{1}{|c|}{\textit{\begin{tabular}[c]{@{}c@{}}Navigate to the refrigerator, grab a beverage\\  and deliver it at the laptop\end{tabular}}} & \multicolumn{1}{c|}{4/4}                & \multicolumn{1}{c|}{0/4}                       & 3/4                     \\ \hline
% \multicolumn{1}{|c|}{\textit{\begin{tabular}[c]{@{}c@{}}Navigate to room 2, grab the cup \\ and water the potted plant\end{tabular}}}                & \multicolumn{1}{c|}{4/5}                & \multicolumn{1}{c|}{0/5}                       & 4/5                     \\ \hline
% \multicolumn{1}{|c|}{\textit{\begin{tabular}[c]{@{}c@{}}Turn off the TV in room 2 \\ and head over the couch\end{tabular}}}                          & \multicolumn{1}{c|}{2/3}                & \multicolumn{1}{c|}{0/3}                       & 3/3                     \\ \hline
% \multicolumn{4}{|c|}{\textbf{ENVIRONMENT 2}}                                                                                                                                                                                                                              \\ \hline
% \multicolumn{1}{|c|}{\textit{Navigate to the garage}}                                                                                                & \multicolumn{1}{c|}{1/1}                & \multicolumn{1}{c|}{0/1}                       & 1/1                     \\ \hline
% \multicolumn{1}{|c|}{\textit{Navigate to the lounge}}                                                                                                & \multicolumn{1}{c|}{1/1}                & \multicolumn{1}{c|}{0/1}                       & 1/1                     \\ \hline
% \multicolumn{1}{|c|}{\textit{Navigate to the Cafe}}                                                                                                  & \multicolumn{1}{c|}{1/1}                & \multicolumn{1}{c|}{0/1}                       & 1/1                     \\ \hline
% \multicolumn{1}{|c|}{\textit{Navigate to the game room}}                                                                                             & \multicolumn{1}{c|}{1/1}                & \multicolumn{1}{c|}{0/1}                       & 0/1                     \\ \hline
% \multicolumn{1}{|c|}{\textit{\begin{tabular}[c]{@{}c@{}}Navigate to the garage to check \\ if the delivery truck is still here\end{tabular}}}        & \multicolumn{1}{c|}{1/1}                & \multicolumn{1}{c|}{0/1}                       & 1/1                     \\ \hline
% \multicolumn{1}{|c|}{\textit{\begin{tabular}[c]{@{}c@{}}Navigate to the cafe, grab a water \\ bottle and drop it off at the lounge\end{tabular}}}    & \multicolumn{1}{c|}{4/5}                & \multicolumn{1}{c|}{0/5}                       & 3/5                     \\ \hline
% \multicolumn{1}{|c|}{\textit{\begin{tabular}[c]{@{}c@{}}Fill the cup in the cafe with water \\ at the sink and water the potted plant\end{tabular}}} & \multicolumn{1}{c|}{5/6}                & \multicolumn{1}{c|}{0/6}                       & 5/6                     \\ \hline
% \multicolumn{1}{|c|}{\textbf{Score}}                                                                                                                 & \multicolumn{1}{c|}{\textbf{26/30}}        & \multicolumn{1}{c|}{\textbf{0/30}}                & \textbf{24/30}             \\ \hline
% \end{tabular}
% \label{tab:llm_comparison}
% \end{table*}


% \begin{table}[]
% \centering
% \begin{tabular}{|c|c|c|c|}
% \hline
% \textbf{Metric}                                            & \textbf{Cloud} & \textbf{Pre-Trained} & \textbf{Fine-Tuned} \\ \hline
% \begin{tabular}[c]{@{}c@{}}Our Prompt\\ Score\end{tabular} & 29/30              & 0/30                     & 24/30                   \\ \hline
% \end{tabular}
% \caption{LLM evaluation comparing the cloud cohere LLM as a baseline to the pre-trained TinyLLama LLM and our Fine-Tuned model. Results are shown for evaluating total correct sub-tasks generated versus the expected sub-tasks given 12 high-level natural language prompts.}
% \label{tab:llm_comparison}
% \end{table}

==> sections/tables_and_figures/latency_experiment_table.tex <==
\begin{table*}[t!]
\caption{\textbf{Working out how the data in this table can be represented differently}Real world results for two simulated environments: a home and office space. The agent is first given tasks to navigate to each of the saved landmarks to build up its knowledge base. Then, using objects placed around the environment the agent is asked to interact with the objects using more complex high level tasks. Results containing latency, total power, RAM utilization and swap utilization are shown for prompting a cohere cloud LLM versus the onboard fine-tuned LLM. During each prompt the LLM successfully generated the subtask(s) and the agent executed the navigation and manipulation based actions.}

\begin{tabular}{cccccc}
\hline

\multicolumn{6}{|c|}{\textbf{Environment 1 (home)}}                                                                                                                                                                                                                                                                                                                      \\ \hline
\multicolumn{1}{|c|}{}                                                                                                                & \multicolumn{2}{c|}{\textbf{Cloud LLM}}                                                        & \multicolumn{1}{c|}{}          & \multicolumn{2}{c|}{\textbf{Onboard Fine-Tuned LLM}}                                           \\ \cline{1-3} \cline{5-6} 
\multicolumn{1}{|c|}{\textbf{Simple Prompt}}                                                                                          & \multicolumn{1}{c|}{\textbf{Latency (s)}}      & \multicolumn{1}{c|}{\textbf{Total Power (W)}} & \multicolumn{1}{c|}{\textbf{}} & \multicolumn{1}{c|}{\textbf{Latency (s)}}      & \multicolumn{1}{c|}{\textbf{Total Power (W)}} \\ \cline{1-3} \cline{5-6} 
\multicolumn{1}{|c|}{Go to the kitchen}                                                                                               & \multicolumn{1}{c|}{0.02}                      & \multicolumn{1}{c|}{6.2}                      & \multicolumn{1}{c|}{}          & \multicolumn{1}{c|}{7.8}                       & \multicolumn{1}{c|}{8.7}                      \\ \cline{1-3} \cline{5-6} 
\multicolumn{1}{|c|}{Go to the kids room}                                                                                             & \multicolumn{1}{c|}{0.02}                      & \multicolumn{1}{c|}{6.2}                    & \multicolumn{1}{c|}{}          & \multicolumn{1}{c|}{7.5}                       & \multicolumn{1}{c|}{9.5}                      \\ \cline{1-3} \cline{5-6} 
\multicolumn{1}{|c|}{Go to the living room}                                                                                           & \multicolumn{1}{c|}{0.03}                      & \multicolumn{1}{c|}{6.2}                      & \multicolumn{1}{c|}{}          & \multicolumn{1}{c|}{7.9}                       & \multicolumn{1}{c|}{9.3}                      \\ \cline{1-3} \cline{5-6} 
\multicolumn{1}{|c|}{\textbf{Complex Prompt}}                                                                                         & \multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{}          & \multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         \\ \cline{1-3} \cline{5-6} 
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}I'm hungry, bring the banana\\ to the laptop\end{tabular}}                            & \multicolumn{1}{c|}{0.01}                      & \multicolumn{1}{c|}{6.2}                      & \multicolumn{1}{c|}{}          & \multicolumn{1}{c|}{13.3}                      & \multicolumn{1}{c|}{9.3 -\textgreater 7.9}    \\ \cline{1-3} \cline{5-6} 
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}My son forgot his teddy bear, \\ take the teddy bear to the kids room.\end{tabular}}  & \multicolumn{1}{c|}{0.02}                      & \multicolumn{1}{c|}{6.2}                      & \multicolumn{1}{c|}{}          & \multicolumn{1}{c|}{16.2}                      & \multicolumn{1}{c|}{9.2 -\textgreater 7.9}    \\ \cline{1-3} \cline{5-6}                                                                                                                                                                                     & \multicolumn{1}{l}{}                           & \multicolumn{1}{l}{}                          & \multicolumn{1}{l}{}           & \multicolumn{1}{l}{}                           & \multicolumn{1}{l}{}                          \\ \hline
\multicolumn{6}{|c|}{\textbf{Environment 2 (office space)}}                                                                                                                                                                                                                                                                                                              \\ \hline
\multicolumn{1}{|c|}{}                                                                                                                & \multicolumn{2}{c|}{\textbf{Cloud LLM}}                                                        & \multicolumn{1}{c|}{}          & \multicolumn{2}{c|}{\textbf{Onboard Fine-Tuned LLM}}                                           \\ \cline{1-3} \cline{5-6} 
\multicolumn{1}{|c|}{\textbf{Simple Prompt}}                                                                                          & \multicolumn{1}{c|}{\textbf{Latency (s)}}      & \multicolumn{1}{c|}{\textbf{Total Power (W)}} & \multicolumn{1}{c|}{\textbf{}} & \multicolumn{1}{c|}{\textbf{Latency (s)}}      & \multicolumn{1}{c|}{\textbf{Total Power (W)}} \\ \cline{1-3} \cline{5-6} 
\multicolumn{1}{|c|}{Go to the lounge}                                                                                                & \multicolumn{1}{c|}{0.01}                     & \multicolumn{1}{c|}{6.2}                      & \multicolumn{1}{c|}{}          & \multicolumn{1}{c|}{8.1}                       & \multicolumn{1}{c|}{8.9}                      \\ \cline{1-3} \cline{5-6} 
\multicolumn{1}{|c|}{Go to the lobby}                                                                                                 & \multicolumn{1}{c|}{0.02}                      & \multicolumn{1}{c|}{6.2}                      & \multicolumn{1}{c|}{}          & \multicolumn{1}{c|}{7.2}                       & \multicolumn{1}{c|}{9.0}                      \\ \cline{1-3} \cline{5-6} 
\multicolumn{1}{|c|}{Go to the office}                                                                                                & \multicolumn{1}{c|}{0.03}                      & \multicolumn{1}{c|}{6.2}                      & \multicolumn{1}{c|}{}          & \multicolumn{1}{c|}{6.7}                       & \multicolumn{1}{c|}{9.1}                      \\ \cline{1-3} \cline{5-6} 
\multicolumn{1}{|c|}{Go to the meeting room}                                                                                          & \multicolumn{1}{c|}{0.01}                      & \multicolumn{1}{c|}{6.2}                      & \multicolumn{1}{c|}{}          & \multicolumn{1}{c|}{7.5}                       & \multicolumn{1}{c|}{9.3}                      \\ \cline{1-3} \cline{5-6} 
\multicolumn{1}{|c|}{\textbf{Complex Prompt}}                                                                                         & \multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{}          & \multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}                         \\ \cline{1-3} \cline{5-6} 
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}I'm feeling lonely, bring the\\  teddy bear to the office\end{tabular}}               & \multicolumn{1}{c|}{0.04}                      & \multicolumn{1}{c|}{6.2}                      & \multicolumn{1}{c|}{}          & \multicolumn{1}{c|}{15.2}                      & \multicolumn{1}{c|}{9.1 -\textgreater{}8.0}   \\ \cline{1-3} \cline{5-6} 
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Guests are here and they are thirsty,\\  bring the bottle to the lobby.\end{tabular}} & \multicolumn{1}{c|}{\textless 0.01}            & \multicolumn{1}{c|}{6.2}                      & \multicolumn{1}{c|}{}          & \multicolumn{1}{c|}{16.2}                      & \multicolumn{1}{c|}{9.3 -\textgreater{}7.6}   \\ \cline{1-3} \cline{5-6}                                                                                                   
\end{tabular}
\label{tab:real_world}
\end{table*}


